Refining 6-DoF Grasps with Context-Specific Classifiers

In this work, we present GraspFlow, a refinement approach for generating context-specific grasps. We formulate the problem of grasp synthesis as a sampling problem: we seek to sample from a context-conditioned probability distribution of successful grasps. However, this target distribution is unknown. As a solution, we devise a discriminator gradient-flow method to evolve grasps obtained from a simpler distribution in a manner that mimics sampling from the desired target distribution. Unlike existing approaches, GraspFlow is modular, allowing grasps that satisfy multiple criteria to be obtained simply by incorporating the relevant discriminators. It is also simple to implement, requiring minimal code given existing auto-differentiation libraries and suitable discriminators. Experiments show that GraspFlow generates stable and executable grasps on a real-world Panda robot for a diverse range of objects. In particular, in 60 trials on 20 different household objects, the first attempted grasp was successful 94% of the time, and 100% grasp success was achieved by the second grasp. Moreover, incorporating a functional discriminator for robot-human handover improved the functional aspect of the grasp by up to 33%.

==> content/relatedwork.tex <==
\section{Background \& Related Work}
Our work pertains to the study of robot grasping, which has a rich history and encompasses a variety of approaches. Here, we provide a brief summary of key related work in data-driven grasp synthesis and context-based grasping. We refer readers desiring more comprehensive information to excellent survey articles~\cite{bohg2013data,shimoga1996robot,sahbani2012overview,kleeberger2020survey}. 

\mypara{Grasp Synthesis.} \hsnote{to rewrite} The objective of grasp synthesis is to obtain a gripper configuration that results in a successful grasp. Success is typically indicated using some quality metrics. Classic analytical approaches can be effective but require precise geometric and physical object models, and do not generalize well to new objects. ``analytic refers to methods that construct force closure grasps with a multi-fingered robotic hand that are dexterous, in equilibrium, stable and exhibit a certain dynamic behaviour.'' Recent data-driven methods have leveraged advances in deep learning to synthesize suitable grasps from low-level observations (e.g., RGB-D or pointclouds) and derive models that generalize to novel  objects~\cite{lenz2015deep,ten2017grasp,mahler2017dex,levine2018learning,satish2019policy,morrison2018closing}. 

Of particular note is GraspNet which applies variational autoencoders towards 6-DOF stable grasp  generation~\cite{mousavian20196}.  
%This work  has been extended for grasping in a clutter~\citep{murali20206}, larger datasets~\citep{eppner2021acronym}, and human-robot handover~\citep{yang2021reactive}. 
Interestingly, GraspNet also refines grasps using the derivative of the grasp evaluator; in fact, this particular instance of refinement is a specific variant of \method{} using the KL-divergence without the diffusion term. However, later works applying GraspNet to grasp in clutter~\cite{murali20206} and for human-robot handover~\cite{yang2021reactive} replaced the gradient-based refinement with a Monte-Carlo sampling approach, citing similar performance with lower cost. However, our experiments show that refinement based on gradient flows can yield far better grasp candidates. In this paper, we provide theoretical motivation underlying the and generalize the approach towards other $f$-divergences and additional contexts beyond stability. As we will see, using \method, it is not necessary to discard grasps that violate robot kinematics~\cite{mousavian20196}. Using the perspective of gradient flows, we are able to construct superior refinement schemes by constructing suitable discriminators. 

\mypara{Context-based and Semantic Grasping.} Grasps are often performed in relation to a desired goal, e.g., tool-use or manipulation. From this broader perspective, analytical properties are desirable but  insufficient: robots require grasps that are \emph{functionally appropriate}~\cite{dang2012semantic}. Recognition of this issue has led to work on generating/selecting grasps that satisfy constraints associated with tasks (e.g., a pouring task requires that the grasp not block the container opening) and other contexts such as object material~\cite{liu2020cage} and target~\cite{sun2021gater}. At a high-level, a typical setup involves learning from labelled data~\cite{murali2020taskgrasp} to associate low-level features and task/object information to semantic constraints. The constraints are often represented by a model (e.g., affordance map~\cite{dang2012semantic}, probabilistic graphical model~\cite{song2010learning}, neural network~\cite{liu2020cage,murali2020taskgrasp}) that is used in planning~\cite{dang2012semantic} or, more commonly, to \emph{rank} grasp candidates that are pre-generated using a context-free stable grasping method. 

\hsnote{need to cite \cite{detry2017task}.}

In contrast to these prior works, \method{} \emph{refines rather than ranks}; it transforms a context-free grasp into one that is context-appropriate. Our focus is \emph{not} to learn semantic constraints; we assume the task-relevant semantics are provided (e.g., using one of the above methods or via affordance-based techniques~\cite{antanas2019semantic}). Our approach mitigates having to iterate over a large number of grasp candidates, none of which may be appropriate. \hsnote{more advantages / differences here}%Instead of having a single ``monolithic'' model, \method{} is modular and enables the semantic context to be composed at run-time, and updated as more data becomes available. 

 \hsnote{need to cite energy based models.}. Our 
 

